Outlier Detection Bias Busted: Understanding Sources of Algorithmic Bias through Data-centric Factors

The astonishing successes of ML have raised growing concern for the fairness of modern methods when deployed in real world settings. However, studies on fairness have mostly focused on supervised ML, while unsupervised outlier detection (OD), with numerous applications in finance, security, etc., have attracted little attention. While a few studies proposed fairness-enhanced OD algorithms, they remain agnostic to the underlying driving mechanisms or sources of unfairness. Even within the supervised ML literature, there exists debate on whether unfairness stems solely from algorithmic biases (i.e. design choices) or from the biases encoded in the data on which they are trained. To close this gap, this work aims to shed light on the possible sources of unfairness in OD by auditing detection models under different data-centric factors. By injecting various known biases into the input data -- as pertain to sample size disparity, under-representation, feature measurement noise, and group membership obfuscation -- we find that the OD algorithms under the study all exhibit fairness pitfalls, although differing in which types of data bias they are more susceptible to. Most notable of our study is to demonstrate that OD algorithm bias is not merely a data bias problem. A key realization is that the data properties that emerge from bias injection could as well be organic -- as pertain to natural group differences w.r.t. sparsity, base rate, variance, and multi-modality. Either natural or biased, such data properties can give rise to unfairness as they interact with certain algorithmic design choices.

==> math_commands.tex <==

\usepackage{amsmath,amsfonts,bm}

\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

\newcommand{\newterm}[1]{{\bf #1}}


\def\figref#1{figure~\ref{#1}}
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
\def\secref#1{section~\ref{#1}}
\def\Secref#1{Section~\ref{#1}}
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
\def\eqref#1{equation~\ref{#1}}
\def\Eqref#1{Equation~\ref{#1}}
\def\plaineqref#1{\ref{#1}}
\def\chapref#1{chapter~\ref{#1}}
\def\Chapref#1{Chapter~\ref{#1}}
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
\def\algref#1{algorithm~\ref{#1}}
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
\def\partref#1{part~\ref{#1}}
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\pdata}{p_{\rm{data}}}
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} %

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} 


\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak




==> theoretical_findings.tex <==

In this section, we derive some theoretical justification of why LoF and iForest can adapt well (or poorly) to different injected biases. We will introduce the mathematical notations, assumptions and background algorithms for various detectors in Appx. \ref{assec:preliminary}, and then provide theoretical results in Appx.\ref{assec:theory_result}.


\subsection{Preliminaries}
\label{assec:preliminary}

\subsubsection{Probability and Outlier Score}
In the main text, we use flag rate $P(O =1| G)$ to measure the fairness of the algorithm. However, our outlier detection algorithms rarely give a direct estimation of the true probability scores. For example, LoF algorithm uses local outlier factor as the outlier score, iForest measures the outlierness by average path lengths of iTrees, and DeepAE outputs the reconstruction score of decoder. Therefore, we first decompose the probability of flagging out a point as outlier $P(O=1)$ as:
\begin{align}
P(O=1) &= P(O=1 |G=a)P(G=a) + P(O=1 |G=b)P(G=b) \\
\nonumber &= \Big[P(O=1 |G=a, Y=1)P(Y=1  G=a)  \\
\nonumber &+ P(O=1 |G=a, Y=0) P(Y=0 |G=a) \Big]P(G=a)  \\
\nonumber &+ \Big[P(O=1 |G=b, Y=1)P(Y=1| G=b) \\ &+ P(O=1 |G=b, Y=0) P(Y=0 |G=b) \Big]P(G=b)
\end{align}

When inlier and outlier samples from both group $a,b$ are equally sampled, $P(G=a)$ and $P(G=b)$ will not change. $P(Y=0|G=i)$, $P(Y=1 |G=i),\forall i \in \{a,b\}$ will also remain the same if we do not change the fraction of outliers within the both groups. During the experiment, each outlier detection algorithm will flag out equal numbers of outliers, making $P(O=1)$ at equal rate throughout our analysis. Therefore, when $P(O=1 |G=i, Y=j)$ for $i \in \{a,b\}$ and $j \in \{0,1\}$ increases, it means that at least one of the other probabilities will decrease. Then, we can relate outlier scores to probability. For points (either inlier points or outlier points) from either protected group $a$ or $b$, if we assign higher outlier scores to the points than points in other groups, it implies that the probability of flagging out the points will increase, with possible decreases in detecting the rest of data points as outliers.  

\subsubsection{Background on LoF}

LoF computes the local density deviation of a given data point with respect to its neighborhood points, and using the ratio of density deviation as the outlier score $S$. The larger $S$ than one indicates that a point is more inclined as outlier with higher $P(O=1|x)$. To compute the local density deviation, one needs to compute the reachability distance. The detailed calculation are provided by the definitions below.

\textit{Definition 1}: \textbf{k-distance}. Assume the distance between two data points is $d(p,o)$, then given a dataset $\mathcal{D}$, for a data $p \in \mathcal{D}$ and a positive integer $k$, $o_k$ is the $k$-th nearest neighborhood point of $p$, the $k$-distance of a data point $p$ is defined as:  
\[\text{k-distance(p)} = d(p,o_k) \]

\textit{Definition 2}: \textbf{Reachability distance}.  Reachability distance (RD) is the distance to travel from a point to its neighbor. For any two data points $p,o \in \mathcal{D}$. The reachability distance is:
\[\text{RD}_k (p,o) = \max (\text{k-distance}(o),d(p,o) )\]

\textit{Definition 3}: \textbf{Local Reachability Density}. For any point $p$, denote the set of $k$-nearest neighbor points by $N_k(p) \subseteq \mathcal{D}$, the local reachability density (LRD) of $p$ is:
\[\text{LRD}_k(p) = \frac{1}{
\sum_{o \in N_k(p)} RD_k (p,o)/ |N_k(p)|
}
\]

\textit{Definition 4}: \textbf{Local Outlier Factor}. The core of LOF algorithm is the calculation of local outlier factor, which measures density deviation of the point to its neighbors. Intuitively, if the factor is closer to $1$, it means that the density factor of the point is similar to the neighbors' densities, suggesting that the point is less anomalous, and vise versa. The local outlier factor of $p$ will be calculated as:

\[\text{LOF}_k(p)= \frac{\sum_{o \in N_k(p)} \text{LRD}_k(o)}{ |N_k(p)| \cdot \text{LRD}_k(p)} \]
Given a dataset $\mathcal{D}$, the local outlier factor algorithm outputs the score $S$ of point $p \in \mathcal{D}$ based on local outlier factor. 

\subsubsection{Background on iForest} iForest considers the average number of steps required to isolate a point from the others. It starts with building iTrees, which makes random threshold cuts sequentially on randomly chosen features. A iTree is complete when until all points are the same for a leaf node, or a leaf node contains only one point. The outlier score of a point is chosen as the average paths of ensembled iTrees to reach one node. 

\textit{Definition 5}. \textbf{Path Length.} $h(p)$ of a point $p \in \mathcal{D}$ is measured by the number of edges $p$ traverses an iTree from the root node until the traversal is terminated at an external node.

\textit{Definition 6}. \textbf{iForest Scores.} For an outlier point $p \in \mathcal{D}$ and $|\mathcal{D}| = n$, the score is calculated with $c(n) = 2H(n - 1) - (2(n-1)/n)$ and $H(i)$ is the harmonic number:
\[S(p, n) = 2^{-\frac{\mathbb{E}[h(p)]}{c(n)}}\]

Observe that $c(n)$ is fixed by the size of dataset, and therefore, an outlier $p$ stands out only when $\mathbb{E}[h(p)]$ (average path length across different iTrees) is small, which indicates that $p$ is easily separated out from rest of the points.

It is difficult to directly estimate the average path length over an ensemble of iTrees, given that each iTree is built upon consecutively splitting on random features and random variables. Similar to Appendix A in \cite{isolation-based}, we show the average depths of the trees are dependent upon distances between points. Assume for one-dimensional setting, $x_0 < x_1 < x_2$ are three points from the univariate distribution, and iForest can make maximum two iTrees out of these three points. iTree A will split between $x_0, x_1$ and then split between $x_1, x_2$. iTree B will split between $x_1,x_2$ and $x_0, x_1$. Then, $P(h(x_0) = 1) = P(h(x_2) = 2) = P(A) = \frac{d(x_0,x_1)}{d(x_0,x_2)}$. $P(h(x_0) = 2) = P(h(x_2) = 1) = P(B) = \frac{d(x_1,x_2)}{d(x_0,x_2)}$. The average path length of $x_1$ is $\mathbb{E}(h(x_1)) = \frac{d(x_0,x_1)}{d(x_0,x_2)} + 2\frac{d(x_1,x_2)}{d(x_0,x_2)}$. Fixed $d(x_0, x_2)$, When $x_0$ is closer to $x_1$ and further away from $x_2$, the average path length grows. On the contrary, when $x_0$ deviates from its neighbor $x_1$, the average path length becomes smaller, suggesting that $x_0$ is more likely to be outliers than $x_1, x_2$. Though not rigorously proven, the above example suggests that a point's outlier score (average path length) is related to the distances to the other points.

\textit{Assumption 1.} The iForest will construct iTrees by splitting among each dimension and each feature values uniformly at random. \label{assumption:iforest}

\textit{Assumption 2.} Given a n-dimensional point $\mathbf{p} \in \mathcal{D}^n$, the average tree length $\mathbb{E}(h(\mathbf{p}))$ is related inverse-proportionally to the pair-wise distances with other points:
\begin{align}
\mathbb{E}(h(\mathbf{p})) &\propto  \frac{1}{\prod_{j=1}^n \mathbb{E}[P(\text{Split between } \mathbf{p}_j \text{ and } \mathbf{p}_j \text{'s neighbors})]} \\
&\propto \prod_{j=1}^n \frac{\max_{\mathbf{q} \in \mathcal{D}} d(\mathbf{q}_j, \mathbf{p}_j)}{ \frac{1}{k} \sum_{ \mathbf{o} \in N_k(\mathbf{p})} d(\mathbf{o}_j, \mathbf{p}_j)}
\end{align}

where $\frac{1}{k} \sum_{ \mathbf{o} \in N_k(\mathbf{p})} d(\mathbf{o}_j, \mathbf{p}_j)$ is the average distance of $\mathbf{p}$ to its $k$-neighbors along $j^\text{th}$ dimension, and $\max_{\mathbf{q} \in \mathcal{D}} d(\mathbf{q}_j, \mathbf{p}_j)$ measures the maximum distance of a point and all points along $j$, which functions as a inlierizing constant. This makes sense, since if a point is of significant distance from the neighbors, the average distance becomes larger and split will be conducted more easily. With larger probability of splitting between the anomalous point and its neighbors, the average path length should be shorter, yielding higher outlier scores. While it is not clear how to find the optimal $k$, we choose $k$ to be the size of inlier/outlier data point groups.




\subsection{Theoretical Analysis on Clustered Outliers}
\label{assec:theory_result}

\subsubsection{Clustered Outliers}
Clustered outliers are small group of points that deviate from the inlier points' distributions. Let $G_{out}$ denotes the outlier cluster and $G_{ind}$ denotes the inlier cluster, we assume the following assumptions hold for cluster outliers: 

\textit{Assumption 3}. outlier clusters may have either larger or smaller densities than inlier clusters. For simplicity of our analysis, we assume clustered Outliers are of the same density of inlier clusters. Let $d_{ab}$ denotes the average intra-distance of outlier cluster and $d_{nor}$ denotes the average intra-distance of inlier cluster, we have:
\[d_{ab} = \frac{1}{\binom{|G_{ab}|}{2}} \sum_{\substack{x,y \in G_{ab} \\ x \neq y}} d(x, y)  = \frac{1}{\binom{|G_{nor}|}{2}} \sum_{\substack{x,y \in G_{nor} \\ x \neq y}} d(x, y) = d_{nor}\] 

\textit{Assumption 4}. Since the clustered Outliers are of different distributions from the inlier points, we assume that they reside far from the inlier clusters. Let average inter-cluster distance, denoted as $d_{inter}$, be calculated as:
\[
\scalebox{0.8}{ 
$d_{inter} = \frac{1}{2} \left( \frac{1}{|G_{ab}| \cdot |G_{nor}|} \sum_{x \in G_{ab}} \sum_{y \in G_{nor}} d(x, y) + \frac{1}{|G_{ab}| \cdot |G_{nor}|} \sum_{x \in G_{nor}} \sum_{y \in G_{ab}} d(x, y) \right)$
}
\]
$d_{inter}$ is larger than intra-cluster distances for both inlier and outlier clusters, we have $d_{inter} > d_{ab}$ and $d_{inter} > d_{nor}$.


\textit{Assumption 5.} Similar to our data simulation setting, we assume the population consists of two protected groups of data with $G_a$ and $G_b$, each group has one associating outlier cluster denote as $G_{ab,a}$, $G_{ab,b}$ and inlier cluster denote as $G_{nor,a}$ and $G_{nor,b}$. When two groups are of equal size, the associated expected inter-cluster distances are $d_{ab,a} = d_{ab,b} = d_{nor,a} = d_{nor,b}$, and expected intra-cluster distances between outlier and inlier clusters within group $a$ and $b$ are both $d_{inter}$. 

\textit{Assumption 6.} When there is density variation in the feature spaces, we assume protected group $b$ becomes sparser with higher intra-cluster distance $d_{ab,b}$ and $d_{nor,b}$. When density heterogeneity occurs, we have $d_{ab,b} > d_{ab,a}$ and $d_{nor,b} 
> d_{nor,a}$.

\textit{Assumption 7.} When group-membership obfuscation biases occur, underprevileged individuals change their $\mathcal{X}_g$ features to lie about certain features/identities. For two protected groups of data $G_a$ and $G_b$, while $G_{ab}$, $G_{nor,a}$ remain unchanged with distances $b_{ab}=b_{nor}$ and $b_{inter}$, due to changes in $\mathcal{X}_g$, Group $b$ data points are dividing into subgroups for both Outliers and inlier points. Assume Group $b$ data points break into $n$ groups $[G_{nor,b,1}...G_{nor,b,n}]$ for inlier cluster and $m$ groups $[G_{ab,b,1}... G_{ab,b,m}]$ for outlier cluster. 

\subsubsection{LOF, Density Variation}
Before providing a thoretical analysis of why LOF favors Group $a$ or $b$ in the presence of biases, we will start by two lemmas, which identify that the number of neighbors,$k$, is crucial for the downstream detection results and is needed to be set properly to capture outlier patterns.

\textit{ \textbf{Lemma 1}: For one inlier cluster and outlier cluster, if local outlier factor algorithm catches all the cluster Outliers, the number of neighbors needs to be chosen that $k > |G_{ab}|$.}

\textit{Proof:}
Assume $k \leq |G_{ab}|$. Then, pick any points $p_{ab} \in G_{ab}$ and $p_{nor} \in G_{nor}$. Both point's average distance to their cluster's neighbors are estimated with intra-cluster distances, $d_{ab}$ and $d_{nor}$, respectively. $p_{ab}$'s average distance to the neighbors within the inlier cluster is estimated as the inter-cluster distance, $d_{inter}$.

Since $d_{inter} > d_{ab}$,  $p_{ab}$'s $k$ nearest neighbors will be points that are closer to $p_{ab}$, which constitute of only Outliers within the cluster. Therefore, We have that $N_k(p_{ab}) \subseteq G_{ab}$. Similarly, $p_{nor}$'s $k$ nearest neighbors will be points that are closer to $p_{nor}$, which constitute of only the inlier points. 

Then, the expectation of local outlier factor of the $p_{ab}$ is:
\begin{align}
\mathbb{E}[
\text{LOF}_k(p_{ab})] &= \mathbb{E} \Bigg [  \frac{\sum_{o \in N_k(p_{ab})} \text{LRD}_k(o)}{ |N_k(p_{ab})| \cdot \text{LRD}_k(p_{ab})} \Bigg] \\  &=  \frac{\sum_{o \in N_k(p_{ab})} \mathbb{E} \big [ \text{LRD}_k(o) \big] }{ k \cdot  \mathbb{E} \big [\text{LRD}_k(p_{ab})\big]} \label{eq:expected_lof} \\
 &= \frac{\sum_{o \in N_k(p_{ab})} \mathbb{E} \big [\frac{1}{\sum_{j \in N_k(o)} \text{RD}_k(o,j)/ |N_k(o)|} \big]}{k \mathbb{E}\big[ \frac{1}{\sum_{m \in N_k(p_{ab})} \text{RD}_k (m,p_{ab})/ |N_k(p_{ab})| } \big]} \\ &= \frac{\sum_{o \in N_k(p_{ab})} \frac{1}{\sum_{j \in N_k(o)} \mathbb{E} [\text{RD}_k(o,j)] / k} }{k  \frac{1}{\sum_{m \in N_k(p_{ab})} \mathbb{E} [\text{RD}_k (m,p_{ab})]/ k } } \\ 
&\approx \frac{k \cdot \frac{1}{ k \cdot d_{ab} / k} }{k  \frac{1}{k \cdot d_{ab}/ k } }  = 1
\end{align}
We can similarly show that expected local outlier factor of the $p_{nor}$ will be around $1$. In which case, the local outlier factor algorithm can fail to detect any $p_{ab}$ due to that both outlier points and inlier points have output scores at 1.

When $|G_{nor}| > k > |G_{ab}|$, the $k$-neighbors of the outlier point $p_{ab}$ must contain some points from the inlier clusters, and that $G_{ab} \subseteq N_k(p_{ab})$. For Eq. \ref{eq:expected_lof}, the local reachability density of neighborhood points (the numerator) will be calculated as: 
\begin{align}
\nonumber  &\sum_{o \in G_{ab}} \frac{1}{\sum_{j \in N_k(o)} \mathbb{E} [\text{RD}_k(o,j)] / k} \\  \nonumber &+ \sum_{m \in N_k(p_{ab})\backslash G_{ab}}  \frac{1}{\sum_{n \in N_k(m)} \mathbb{E} [\text{RD}_k(m,n)] / k} \\ = &\sum_{o \in G_{ab}} \frac{1}{d_{inter}} + \sum_{m \in N_k(p_{ab})\backslash G_{ab}} \frac{1}{ 
 d_{nor}} = \frac{ |G_{ab}|} {d_{inter}} + \frac{k-|G_{ab}|}{d_{ab}} 
\end{align}
The last equality holds because that $d_{nor} = d_{ab}$ (Assumption 5). The denominator in Eq. \ref{eq:expected_lof}, the local reachability density of the $p_{ab}$ will be calculated as:
\begin{align}
&k \frac{1}{\sum_{m \in N_k(p_{ab})} \mathbb{E} [\text{RD}_k (m,p_{ab})]/ k } \\
 &=   \frac{k}{\sum_{m \in G_{ab}} \mathbb{E} [\text{RD}_k (m,p_{ab})]/k  + \sum_{n \in N_k(p_{ab}) \backslash G_{ab}} \mathbb{E} [\text{RD}_k (n,p_{ab})] /k} \label{eq:RD_distance_inlier_outlier} \\ 
 &= \frac{k}{|G_{ab}| \cdot d_{inter}/k + (k-|G_{ab}|) \cdot d_{inter}/k} = \frac{k}{d_{inter}}
 \label{eq:denominator}
\end{align}

In Eq. \ref{eq:RD_distance_inlier_outlier}, for both outlier or inlier points, the reachability distance with $p_{ab}$ will always be $d_{inter}$, because k-distance is the furthest reachable point for the k-neighbors, which will be a point from the other cluster. Therefore, the expected outlier factor distance is:
\begin{align}
\mathbb{E}[
\text{LOF}_k(p_{ab})] = \frac{\frac{ |G_{ab}|} {d_{inter}} + \frac{k-|G_{ab}|}{d_{ab}} }{ \frac{k}{d_{inter}}} > 1
\end{align}

Because $k$ is small than $|G_{nor}|$, for any inlier points $p_{nor}$ the expected score will still remain roughly at 1. Then, $p_{ab}$ will be detected at higher outlier scores when $|G_{nor}| > k > |G_{ab}|$.

\textit{\textbf{Lemma 2}: Consider multiple outlier clusters $G_{ab,1}$, $G_{ab,2}$... $G_{ab,k}$ and one inlier cluster $G_{nor}$, if Assumption 3-5 holds, with the average intra-cluser distance in outlier clusters and inlier cluster remain at $d_{ab}$, $d_{nor}$, and the average inter-cluster distance between outlier clusters and inlier cluster remains at $d_{inter}$. For local outlier factor algorithm to catch the cluster Outliers, the number of neighbors $k > \max(|G_{ab,1}|,..., |G_{ab,k}|)$.}

\textit{Proof}: Based on Lemma 1, in order to detect all Outliers from cluster $G_{ab,i}$, we need $k > |G_{ab,i}|$, therefore, $k$ must be larger than sizes of all clusters, and $k > \max(|G_{ab,1}|,..., |G_{ab,k}|)$.

Next, we derive the Proposition 1, which explains LOF's masking effect on Group $b$ because of sparsity in both inlier and outlier clusters. When the masking effect occurs, LOF will prioritize the detection of Group $a$'s Outliers.

\textit{\textbf{Proposition 1}: With density variation in the feature spaces, when $d_{ab,b} > \frac{(k-|G_{ab,b}|)d_{ab,a}}{k-|G_{ab,a}|}$, LOF algorithm will favor labeling group $a$, increasing flag rate $P(O=1|G=a)$. When outlier cluster distance becomes equal to inter-cluster distance between outlier cluster and inlier cluster, $d_{ab,b} = d_{inter}$, downstream performance will drop because of missing outlier points in Group $b$.}


\textit{Proof}:
Based on Lemma 2, we have that the hyper-parameter $k > |G_{ab,a}|$ and $ k > |G_{ab,b}|$.
For an outlier point $p_{ab,i} \in G_{ab,i}$ $i \in \{a,b\}$, we calculate the average local outlier factor is:
\begin{align}
\mathbb{E}[
\text{LOF}_k(p_{ab,i})] &= \mathbb{E} \Bigg [  \frac{\sum_{o \in N_k(p_{ab,i})} \text{LRD}_k(o)}{ |N_k(p_{ab,i})| \cdot \text{LRD}_k(p_{ab,i})} \Bigg] \\  &=  \frac{\sum_{o \in N_k(p_{ab,i})} \mathbb{E} \big [ \text{LRD}_k(o) \big] }{ k \cdot  \mathbb{E} \big [\text{LRD}_k(p_{ab,i})\big]} \\ 
 &= \frac{\sum_{o \in G_{ab,i}} \frac{1}{\sum_{j \in N_k(o)} \mathbb{E} [\text{RD}_k(o,j)] / k} }{k \cdot  \mathbb{E} \big [\text{LRD}_k(p_{ab,i})\big]}  \\ \nonumber &+ \frac{ \sum_{m \in N_k(p_{ab})\backslash G_{ab,i}}  \frac{1}{\sum_{n \in N_k(m)} \mathbb{E} [\text{RD}_k(m,n)] / k} }{k \cdot  \mathbb{E} \big [\text{LRD}_k(p_{ab,i})\big]} \\
&= \frac{\frac{|G_{ab,i}|}{d_{inter}} + \frac{k - |G_{ab,i}|}{d_{ab,i}}}{\frac{k}{d_{inter}}}
\end{align}

For a point $p_{ab,a} \in G_{ab,a}$ (an outlier point from Group $a$) and a point $b_{ab,b} \in G_{ab,b}$ (an outlier point from less dense Group $b$), when $d_{ab,b} > \frac{(k-|G_{ab,b}|)d_{ab,a}}{k-|G_{ab,a}|}$, we have that,
\begin{align}
 \frac{|G_{ab,a}|}{d_{inter}} + \frac{k - |G_{ab,a}|}{d_{ab,a}} -\Bigg( \frac{|G_{ab,b}|}{d_{inter}} + \frac{k - |G_{ab,b}|}{d_{ab,b}} \Bigg) &>0 \\
 \mathbb{E}[
\text{LOF}_k(p_{ab,a})] - \mathbb{E}[\text{LOF}_k(p_{ab,b})] &> 0 
\end{align}

 Therefore, the outlier points from Group $a$ will be flagged out with higher average local outlier factor (outlier) scores. The above inequality shows that when there is density variation within the data groups, LoF algorithm will favor more points from group $a$ to be picked up, as $d_{ab,b}$ passes a threshold value. 
 
 For flag rate $P(O= 1| G=a) = P(O=1|G=b,Y=1)P(Y=1|G=b) +P(O=1|G=b,Y=0)P(Y=0|G=b)$, since $P(O=1|G=b,Y=1)$ increases with higher outlier scores, the flag rate will also increase, showing that LoF algorithm favors detecting Group $a$ Outliers.

 When $d_{ab,b} = d_{inter}$, and group $b$ will become completely indistinguishable for outlier and outlier clusters, an outlier point will have average local outlier factor: 
 \begin{align}
\mathbb{E}[
\text{LOF}_k(p_{ab,b})] &= \frac{\frac{|G_{ab,b}|}{d_{inter}} + \frac{k - |G_{ab,b}|}{d_{inter}}}{\frac{k}{d_{inter}}} = 1
\end{align}

Then, an outlier point in Group $b$ is indistinguishable from inlier points and LoF will assign low outlier score, excoriating the downstream detection performance.  \qedsymbol{}

\subsubsection{iForest, Density Variation} Due to density disparities between groups, the outlier points from $G_{ab,b}$ have larger intra-cluster distance $d_{ab,b}$ than the Outliers from $G_{ab,a}$, making the required path lengths of iTrees shorter to separate out the Outliers in Group $b$. Thus, iForest will bias towards Group $b$ Outliers. 

\textit{\textbf{Proposition 2:} For cluster Outliers, density variation makes the average paths length $\mathbb{E}(h(p_{ab,b}))$ shorter than $\mathbb{E}(h(p_{ab,a}))$ for outlier point $p_{ab,b} \in G_b$. When the average intra-distance of $d_{nor,b}$ is larger than average intra-distance of $d_{ab,a}$, the average paths length to identify a inlier point from Group $b$ is shorter than $\mathbb{E}(h(p_{ab,a}))$. The flag rate $P(O=1 |G=b)$ increases since iForest assigns higher outlier scores to both inlier and outlier points in Group $b$.} 

\textit{Proof:} For simplicity of calculation, let us first assume that outlier and inlier points lie in 1-dimension. Based on Assumption 1 and 2, the average path length of a point $p_{ab,i} \in G_{ab,i}$ for $i \in \{a,b\}$ could be approximated as:
\begin{align}
\mathbb{E}(h(p_{ab,i})) &\propto \frac{\max_{q \in G_{a} \cup G_{b}} d(q, p_{ab,i})}{ \frac{1}{|G_{ab,i}|} \sum_{ o \in G_{ab,i}} d(o, p)} \\
&\propto \frac{\max_{q \in G_{a} \cup G_{b}} d(q, p_{ab,i})}{  d_{ab,i}  } 
\end{align}

When there is density discrepancy between groups (Assumption 6), the average intra-cluster distances $d_{ab,b}$ and $d_{nor,b}$ become larger than $d_{ab,a}$ and $d_{nor,a}$, the average intra-cluster distances of Group $a$. Since only the density of two groups are varied, the maximum distance of data point to the other points, $\max_{q \in G_{a} \cup G_{b}} d(q, p_{ab,i})$ is roughly fixed.

When $d_{ab,b} > d_{ab,a}$, we have:
\begin{align}
\frac{\max_{q \in G_{a} \cup G_{b}} d(q, p_{ab,a})}{d_{ab,a}} &> \frac{\max_{q \in G_{a} \cup G_{b}} d(q, p_{ab,b})}{d_{ab,b}} \\
\mathbb{E}(h(p_{ab,a})) &> \mathbb{E}(h(p_{ab,b}))
\end{align}


The average path lengths taken by an outlier point $p_{ab,b}$ from Group $b$ will be shorter than an outlier point $p_{ab,a}$ from Group $a$. Consequently, we have group $b$ Outliers with higher scores than group $a$ Outliers, and $P(O=1|G=b,Y=1) > P(O=1 |G=a,Y=1)$. 

When the average intra-distance of $d_{nor,b}$ is larger than average intra-distance of $d_{ab,a}$. The average paths length to identify $p_{nor,b} \in G_{nor,b}$ the inlier cluster of group $b$ is:
\begin{align}
\mathbb{E}(h(p_{nor,b})) 
&\propto \frac{\max_{q \in G_{a} \cup G_{b}} d(q, p_{nor,b})}{  d_{nor,b}  } 
\end{align}

is shorter than $\mathbb{E}(h(p_{ab,a}))$, resulting on iForest algorithm to falsely label points in inlier cluster of Group $b$ as Outliers, with $P(O=1|G=b,Y=0) > P(O=1 |G=a,Y=1)$. The flag rate $P(O=1 |G=b)$ increases with both conditionals $P(O=1 |G=b,Y=0)$ and $P(O=1 |G=b,Y=1)$ increase.

Extending to multi-dimensional setting for n-dimensional point $\mathbf{p}_{ab,i} \in G_{ab,i}$, if along each dimension, the average intra-group distance remains at $d_{ab}$, the expected average path length for multi-dimensional point $\mathbf{p}_{ab,i}$ is:
\begin{align}
\mathbb{E}(h(\mathbf{p}_{ab,i})) 
&\propto \prod_{j=1}^n  \frac{\max_{\mathbf{q} \in G_{a} \cup G_{b}} d(\mathbf{q}_j, [\mathbf{p}_{ab,i}]_j)}{  (d_{ab,i})^n  } 
\end{align}

Since $d_{ab,b} > d_{ab,a}$, the differences of distance between points will be more apparent in the n-dimensional setting, with larger differences between $(d_{ab,b})^n$ and  $(d_{ab,a})^n$. We would observe iForest to favor group $b$ more in higher-dimensions by assigning $\mathbf{p}_{ab,b}$ with higher outlier scores. \qedsymbol{}

\subsubsection{LOF, Group-membership Obfuscation}
From Table \ref{tab:summary}, we see that LoF algorithm is one of the most susceptible algorithms to group-membership obfuscation bias in clustered Outliers setting. Not only will LoF overly flag Outliers in group $b$, it will also falsely flagging out inlier points within sub-clusters, deteriorating the detection performance.

\textit{\textbf{Proposition 3}: When group-membership obfuscation bias occurs in Group $b$, any points $p_{ab,b,i}$ from sub-cluster $i$ in Group $b$ will have a higher average local outlier factor score than outlier points from non-obfuscated of Group $a$. Furthermore, when a inlier sub-cluster $j$ from Group b has $|G_{nor,b,j}| < |G_{ab,a}|$, LoF will falsely flag out inlier points within the sub-cluster $j$.}


\textit{Proof}: For simplicity, we assume each subgroup will maintain the average intra-cluster distance $d_{ab} = d_{nor}$, and average inter-cluster distance $d_{inter}$. However, altering certain group's inter- and intra- cluster distance can cause one group to have lower/higher local outlier factors scores, thus further complicating the detection performance and equality among groups.

Based on Lemma 2, we see that hyperparameter $k > |G_{ab,a}| = |G_{ab,b}|$. For an outlier point $p_{ab,b,i}$ in subgroup $i \in [1,..m]$ of $G_b$, the average local reachability density of the point will remain at $\frac{k}{d_{inter}}$ by the same calculation as Eq. \ref{eq:denominator}.

However, for $p_{ab,b,i}$, the local reachability density of its $k$ neighborhood will be instead calculated as: 
$\frac{|G_{ab,b,i}|}{d_{inter}} + \frac{k - |G_{ab,b,i}|}{d_{ab}}$. In comparison to an outlier point $p_{ab,a}$ from group $a$, the point $p_{ab,b,i}$ has fewer neighbors within the current cluster ($|G_{ab,i,b}| < |G_{ab,a}|$). Therefore,for the average local outlier factors between the points, we can derive the following inequality:
\begin{align}
\frac{|G_{ab,a}| - |G_{ab,b,i}|}{d_{ab}} &> \frac{|G_{ab,a}| - |G_{ab,b,i}|}{d_{inter}} \\
\frac{\frac{|G_{ab,b,i}|}{d_{inter}} + \frac{k - |G_{ab,b,i}|}{d_{ab}}}{\frac{k}{d_{inter}}} &>\frac{\frac{|G_{ab,a}|}{d_{inter}} + \frac{k - |G_{ab,a}|}{d_{ab}}}{\frac{k}{d_{inter}}} \\
\mathbb{E}[
\text{LOF}_k(p_{ab,b,i})] &> \mathbb{E}[\text{LOF}_k(p_{ab,a})] 
\end{align}
which demonstrates that points in sub-clusters of group $b$ will be flagged out with a higher outlier score.
Furthermore, if a inlier cluster $G_{nor,b,j}, j \in \{1,...m\}$ has size $|G_{nor,b,j}| < k$, any point $p_{nor,b,j}$ in that inlier sub-cluster  will have the average local outlier factor as:
\begin{align}
\mathbb{E}[
\text{LOF}_k(p_{nor,b,j})]
= \frac{\frac{|G_{nor,b,j}|}{d_{inter}} + \frac{k - |G_{nor,b,j}|}{d_{ab}}}{\frac{k}{d_{inter}}} 
\end{align}

 When $|G_{nor,b,j}| < |G_{ab,a}|$, the inlier point $p_{nor,b,j}$ would have a higher average local outlier factor than a point from the outlier cluster $G_{ab,a}$. Therefore, LoF algorithm's detection performance drops as $P(O=1 | G=b,Y=0)$ and $P(O=1 |G=b, Y=1)$ both increase and LoF falsely flag out sub-cluster points from inlier distributions in Group $b$. \qedsymbol{}

\subsubsection{iForest, Group-membership Obfuscation} Membership obfuscation biases can cause iForest to bias towards protected group $b$, but do not play an strong effect in deteriorating the detection performance, as shown in Table \ref{tab:summary}.

\textit{Proof}: For group-membership obfuscation biases occur, members in $G_b$ randomly change the features in $\mathcal{X}_g$, creating subgroups that deviating from rest of the clusters along the dimensions of $\mathcal{X}_g$. When outlier point $p_{ab,b}$ is changed in subsets of $\mathcal{X}_g$, it is separated out from other Outliers, increasing its average distance $[d_{ab,b}]_j$ to the other Outliers for $j \in \mathcal{X}_g$. The outlier score for $p_{ab_b}$ will increase as a result, since the average path length decrease with the following calculation:
\begin{align}
\nonumber
\mathbb{E}(h(p_{ab,b})) 
&\propto \prod_{j \in \mathcal{X}_o}  \frac{\max_{\mathbf{q} \in G_{a} \cup G_{b}} d(\mathbf{q}_j, [\mathbf{p}_{ab,b}]_j)}{  [d_{ab,b}]_j^ {|\mathcal{X}_o|} } \\ \nonumber &\cdot \prod_{f \in \mathcal{X}_c}  \frac{\max_{\mathbf{q} \in G_{a} \cup G_{b}} d(\mathbf{q}_f, [\mathbf{p}_{ab,b}]_f)}{  [d_{ab,b}]_f^ {|\mathcal{X}_c|} } \\ \nonumber &\cdot \prod_{h \in \mathcal{X}_g}  \frac{\max_{\mathbf{q} \in G_{a} \cup G_{b}} d(\mathbf{q}_l, [\mathbf{p}_{ab,b}]_l)}{  [d_{ab,b}]_l^ {|\mathcal{X}_g|} }
\end{align}

However, when a inlier point $p_{nor,b} \in G_{b}$ changes a subset of features in $\mathcal{X}_g$, its outlier score may not necessarily increase. This is because that a point's average path length of iTrees is influenced by how easily that outlier point is picked out by outlying features $\mathcal{X}_c$ alone. If a inlier point still maintains a relatively small average distance to its neighborhood points $[d_{nor,b}]_f, \forall f \in \mathcal{X}_c$, but only changes $[d_{nor,b}]_l$ for some $l \in \mathcal{X}_g$, its average path length $\mathbb{E}(h(p_{nor,b}))$ will not be shorter than any outlier points $p_{ab,a}$ and $p_{ab,b}$ from both group $a$ and $b$. Therefore, after ranking the outlier points based on average path length, iForest's downstream detection performance is not affected significantly.  



\subsection{Theoretical Analysis on Scattered Outliers}


\subsubsection{Scattered Outliers}
Scattered Outliers are data points that float around the inlier data' distributions. Let $G_{ab}$ denotes the group of outlier points and $G_{nor}$ denotes the group of inlier points. 

\textit{Assumption 7.} Assume the average intra-distance of outlier group $d_{ab} = \frac{1}{\binom{|G_{ab}|}{2}} \sum_{\substack{x,y \in G_{ab} \\ x \neq y}} d(x, y)$, is larger than intra-distance of inlier cluster $d_{nor} = \frac{1}{\binom{|G_{nor}|}{2}} \sum_{\substack{x,y \in G_{nor} \\ x \neq y}} d(x, y)$.  

\textit{Assumption 8}. The average inter-group distance , $d_{inter} = \frac{1}{2} \Big(\frac{1}{|G_{ab}| \cdot |G_{nor}|}$ $\sum_{x \in G_{ab}} \sum_{y \in G_{nor}} d(x, y) + \frac{1}{|G_{ab}| \cdot |G_{nor}|} \sum_{x \in G_{nor}} \sum_{y \in G_{ab}} d(x, y) \Big)$, is larger than intra-distance of inlier points $d_{nor} = \frac{1}{\binom{|G_{nor}|}{2}} \sum_{\substack{x,y \in G_{nor} \\ x \neq y}}$ $d(x, y)$, and is larger than intra-distance among the outlier group $d_{ab}$.

\textit{Assumption 9}. For scattered Outliers, we can not guarantee that the hyperparameter $k$ needs to be chosen to be larger than the size of the outlier group, $|G_{ab}|$. However, when running local outlier factor algorithms within the scattered outlier settings, $k$ is usually picked at a larger number than $|G_{ab}|$, which achieves the best downstream detection performance (highest AUROC).

\subsubsection{LOF}
\textit{\textbf{Proposition 5.} For scattered Outliers, sample size disparity in protected group $b$ will increase the average intra-group distance of Group $b$, and when $d_{ab,b} > \frac{(k-|G_{ab,b}|)d_{ab,a}}{k-|G_{ab,a}|}$,LOF algorithm will favor labeling group $a$. Different from clustered outlier setting, for scattered Outliers, the downstream performance of LOF may not be significantly impacted by the sample size biases. }

\textit{Proof:} For a point $p_{ab,i} \in G_{ab,i}$ $i \in \{a,b\}$, the average local outlier factor is:
\begin{align}
\nonumber
\mathbb{E}[
\text{LOF}_k(p_{ab,i})] &= \mathbb{E} \Bigg [  \frac{\sum_{o \in N_k(p_{ab,i})} \text{LRD}_k(o)}{ |N_k(p_{ab,i})| \cdot \text{LRD}_k(p_{ab,i})} \Bigg] \\ \nonumber &=  \frac{\sum_{o \in N_k(p_{ab,i})} \mathbb{E} \big [ \text{LRD}_k(o) \big] }{ k \cdot  \mathbb{E} \big [\text{LRD}_k(p_{ab,i})\big]} \\ 
\nonumber &= \frac{\sum_{o \in G_{ab,i}} \frac{1}{\sum_{j \in N_k(o)} \mathbb{E} [\text{RD}_k(o,j)] / k}}{k \cdot  \mathbb{E} \big [\text{LRD}_k(p_{ab,i})\big]} \\ \nonumber &+ \frac{\sum_{m \in N_k(p_{ab})\backslash G_{ab,i}}  \frac{1}{\sum_{n \in N_k(m)} \mathbb{E} [\text{RD}_k(m,n)] / k} }{k \cdot  \mathbb{E} \big [\text{LRD}_k(p_{ab,i})\big]}  \\
&= \frac{\frac{|G_{ab,i}|}{\max(d_{ab,i},d_{inter})} + \frac{k - |G_{ab,i}|}{d_{nor,i}}}{\frac{k}{\max(d_{ab,i},d_{inter})}}
\end{align}

Similar to cluster Outliers scenario, data points from Group $a$ could be flagged out with higher local outlier factor scores, due to more disparity between Outliers' and inlier points' local reachability density. However, when $d_{nor,b}= d_{inter}$, $d_{ab,b}$ will frequently grow to larger values than $d_{inter}$ (due to sparsity of Outliers), and therefore, local outlier factor can yield better performances to detect scattered Outliers with group sample size bias.

\textit{\textbf{Proposition 6}: Group-membership obfuscation bias in Group $b$ will cause LOF algorithm to increase $P(O=1 |G = b)$. However, for scattered Outliers, the downstream detection performance is less affected by group-membership obfuscation bias.}

\textit{Proof:} Similar to cluster Outliers, we assume that scattered outlier groups and inlier groups are further divided into sub-groups. In the same as Proposition 2, We can demonstrate that points in subclusters of group $b$ will be flagged out with a higher outlier score. But for sub-group inlier points, since the intra-cluster distances $d_{nor}$ is denser than outlier sub-groups with $d_{ab}$, they are less likely to be called out as Outliers, making local outlier factor algorithm relatively robust in this scenario.

\subsubsection{iForest}
For scattered Outliers, sample size biases will also cause iForest to bias towards protected group $b$. iForest is susceptible to sample size biases in scattered Outliers, displaying a decrease in downstream detection accuracy. Although still biasing towards protected group $b$, iForest is more robust to membership obfuscation biases in detecting scattered Outliers. The proofs for the two observations are similar to Proposition 3 and Proposition 4. 



